BLIP: Facilitating the Exploration of Undesirable Consequences of Digital Technologies

Digital technologies have positively transformed society, but they have also led to undesirable consequences not anticipated at the time of design or development. We posit that insights into past undesirable consequences can help researchers and practitioners gain awareness and anticipate potential adverse effects. To test this assumption, we introduce BLIP, a system that extracts real-world undesirable consequences of technology from online articles, summarizes and categorizes them, and presents them in an interactive, web-based interface. In two user studies with 15 researchers in various computer science disciplines, we found that BLIP substantially increased the number and diversity of undesirable consequences they could list in comparison to relying on prior knowledge or searching online. Moreover, BLIP helped them identify undesirable consequences relevant to their ongoing projects, made them aware of undesirable consequences they "had never considered," and inspired them to reflect on their own experiences with technology.

==> sections/list/keywords.tex <==
\begin{itemize}[leftmargin=0.15in]
    \item \textbf{Social Media}: \texttt{social media}\footnote{We avoided product-specific search terms to avoid capturing generic articles that included text, such as ``Share this link on Facebook and Twitter''.}
    \item \textbf{Voice Assistants}: \texttt{voice assistant, chatbot, home assistant, AI assistant, speech recognition, voice recognition, smart assistant, personal assistant}
    \item \textbf{Virtual Reality}: \texttt{virtual reality, mixed reality, augmented reality, metaverse}
\end{itemize}

==> sections/tables/perf-aspect.tex <==
%  \begin{table}[h]
%   \caption{Performance of Aspect Classifiers}
% \label{tab:perfaspect}
%  \small
%  \begin{tabular}{lcccc}
%  \toprule
%  \textbf{Attribute Classifier} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} & \textbf{Acc.} \\
%  \midrule
% Random & 0.09 & 0.11 & 0.09 & 0.11 \\
% \hdashline[1.5pt/5pt]\noalign{\vskip 0.07cm}
% NLI (zero-shot) & 0.31 & 0.34 & 0.30 & 0.36 \\
% \textbf{GPT-3 (zero-shot, ours)} & \textbf{0.38} & \textbf{0.34} & \textbf{0.36} & \textbf{0.38} \\
% \bottomrule
%  \end{tabular}
%  \end{table}

 \begin{table}[h]
  \caption{Performance of Aspect Classifiers}
\label{tab:perfaspect}
 \small
 \begin{tabular}{lcc}
 \toprule
 \textbf{Attribute Classifier} & \textbf{F1} & \textbf{Acc.} \\
 \midrule
Random & 0.09 & 0.11 \\
\hdashline[1.5pt/5pt]\noalign{\vskip 0.07cm}
NLI (zero-shot) & 0.30 & 0.36 \\
\textbf{gpt-3.5-turbo (zero-shot, ours)} & \textbf{0.36} & \textbf{0.38} \\
\bottomrule
 \end{tabular}
 \end{table}

==> sections/tables/perf-filter.tex <==

%  \begin{table}[h]
%   \caption{Performance of Filters}
%  \label{tab:perffilter}
%  \Description{Table contains six columns with the headers Relevance Classifier, Labels, Precision, Recall, F1, and Accuracy. The maximum precision is 0.68, the maximum recall is 0.97, and the maximum F1 score and Accuracy are 0.77 and 0.64, respectively.}
%  \small
%  \begin{tabular}{lcccc}
%  \toprule
%  \textbf{Title Classifier} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} & \textbf{Acc.} \\
%  \midrule
%  Title [always irrelevant] & 0.00 & 0.00 & 0.00 & 0.61
% \\[0.07cm]
% \hdashline[1.5pt/5pt]\noalign{\vskip 0.07cm}
% NLI (zero-shot) & 0.52 & 0.37 & 0.43 & 0.62 \\
% RoBERTa (supervised) & \textbf{0.87} & \textbf{0.86} & \textbf{0.87} & \textbf{0.87} \\
% \bottomrule
%  \end{tabular}
%  \end{table}

 \begin{table}[h]
  \caption{Performance of Filters}
 \label{tab:perffilter}
 \Description{Table contains six columns with the headers Relevance Classifier, Labels, Precision, Recall, F1, and Accuracy. The maximum precision is 0.68, the maximum recall is 0.97, and the maximum F1 score and Accuracy are 0.77 and 0.64, respectively.}
 \small
 \begin{tabular}{lcc}
 \toprule
 \textbf{Relevance Classifier} & \textbf{F1} & \textbf{Acc.} \\
 \midrule
 Title [always irrelevant] & 0.00 & 0.61
\\[0.07cm]
\hdashline[1.5pt/5pt]\noalign{\vskip 0.07cm}
NLI (zero-shot) & 0.43 & 0.62 \\
RoBERTa (supervised) & 0.87 & 0.87 \\
\textbf{gpt-3.5-turbo (zero-shot, ours)} & \textbf{0.90} & \textbf{0.89} \\
\bottomrule
 \end{tabular}
 \end{table}
